Fair and Efficient Allocation of Indivisible Chores with Surplus

We study fair division of indivisible chores among $n$ agents with additive disutility functions. Two well-studied fairness notions for indivisible items are envy-freeness up to one/any item (EF1/EFX) and the standard notion of economic efficiency is Pareto optimality (PO). There is a noticeable gap between the results known for both EF1 and EFX in the goods and chores settings. The case of chores turns out to be much more challenging. We reduce this gap by providing slightly relaxed versions of the known results on goods for the chores setting. Interestingly, our algorithms run in polynomial time, unlike their analogous versions in the goods setting. We introduce the concept of $k$ surplus which means that up to $k$ more chores are allocated to the agents and each of them is a copy of an original chore. We present a polynomial-time algorithm which gives EF1 and PO allocations with $(n-1)$ surplus. We relax the notion of EFX slightly and define tEFX which requires that the envy from agent $i$ to agent $j$ is removed upon the transfer of any chore from the $i$'s bundle to $j$'s bundle. We give a polynomial-time algorithm that in the chores case for $3$ agents returns an allocation which is either proportional or tEFX. Note that proportionality is a very strong criterion in the case of indivisible items, and hence both notions we guarantee are desirable.

==> EF1-PO.tex <==
\section{EF1 + \lowercase{f}PO + Charity} \label{ef1-sec}

In this section, we prove that after introducing at most $n-1$ chores, an allocation exists which is EF1 and fPO at the same time. Each of these new chores is a copy of an existing chore. The high-level idea is to first consider a fractional allocation $x$ which admits a CEEI. Then to each agent, we fully allocate some of the chores that are fractionally allocated to her in $x$. This way, each agent is only receiving her MPB chores and therefore the allocation is fPO. Furthermore, we guarantee that each agent earns at least $1$ unit of money and there exists a chore that upon its removal, the earned money drops below $1$. This way, we can also guarantee EF1 property for the allocation. In order to achieve such an allocation, we allocate some chores to multiple agents and hence we need multiple copies of some of the chores. However, we prove that the number of required copies does not exceed $n-1$. Basically, our algorithm introduces at most $n-1$ copies of the existing chores and finds an integral Fisher equilibrium where each agent earns $1$ unit of money up to one chore.

Given an instance $\mathcal{I} = \langle [n], M, \mathcal{D} \rangle$, let $\langle p,x \rangle$ be a CEEI such that the allocation graph of $x$ is acyclic. By Proposition \ref{acyclic-prop} such an allocation exists. Each of the connected components of the graph is a tree. For each of the trees $T$ do the following. Take an arbitrary agent $i_0$ in $T$ and consider $T$ rooted at $i_0$. Let $X_i$ be the set of chores that are fractionally (or fully) allocated to agent $i$, i.e., $X_i = \{c \in M | x_{i,c} > 0\}$. We introduce the integral allocation $Y$ as follows. For each agent $i$, first we allocate all chores that are fully allocated to her in $x$, i.e., $Y_i \leftarrow \{c \in M | x_{i,c} = 1\}$. For agent $i_0$, as long as $p(Y_{i_0}) < 1$, we keep adding chores from $X_{i_0} \setminus Y_{i_0}$ to $Y_{i_0}$. Since $p(X_{i_0}) \geq 1$, this procedure terminates. Then we iterate on the agents in $T$ in a breadth-first order and for each agent $i$ we do the following. Let $c_i$ be the chore corresponding to the parent of agent $i$ in $T$. If $c_i$ is not allocated yet, we add it to $Y_i$, i.e., $Y_i \leftarrow Y_i \cup \{c_i\}$. Then, we keep adding the chores in $X_i \setminus (Y_i \cup \{c_i\})$ to $Y_i$ until $p(Y_i) \geq 1$ or we run out of chores. Note that all chores in $X_i \setminus (Y_i \cup \{c_i\})$ correspond to children nodes of agent $i$ in $T$. If at the end of this process $p(Y_i) < 1$, we also add a copy of $c_i$ to $Y_i$. Algorithm \ref{existence-alg} shows the pseudocode of our algorithm. In the rest of this section we prove that allocation $Y$ is pEF1 and fPO with at most $(n-1)$ charity. 

\begin{algorithm} 
	\caption{EF1 + fPO + $(n-1)$ charity} \label{existence-alg}
	\begin{algorithmic}
	    \State Input : Instance $\mathcal{I} = ([n], M, \mathcal{D})$
	    \State Output: Allocation $Y$ 
	
	    \State $\langle x, p \rangle \leftarrow$ CEEI($\mathcal{I}$)
	    \For {$i \in [n]$}
	        \State $X_i \leftarrow \{c \in M | x_{i,c} > 0\}$
	        \State $Y_i \leftarrow \{c \in M | x_{i,c} = 1\}$ 
	    \EndFor
	    \For{all connected components $T$ of allocation graph of $x$}
    	    \State $\backslash \backslash$ Let $T$ be rooted at $i_0$
	        \For{all agents $i$ in $T$ in BFS-order}
	            \If {$i \neq i_0$}
	                $c_i \leftarrow$ parent chore of $i$ in $T$
    	        \EndIf
	            \If{$c_i$ is not allocated}
	                \State $Y_i \leftarrow Y_i \cup \{c_i\}$
	            \EndIf
    	        \For{$c \in X_i \setminus (Y_i \cup \{c_i\})$}
	                \If {$p(Y_i) < 1$}
	                    \State $Y_i \leftarrow Y_i \cup \{c\}$
	                \EndIf
	            \EndFor
    	        \If {$p(Y_i) < 1$}
	                \State $Y_i \leftarrow Y_i \cup \{c_i\}$
	            \EndIf
	        \EndFor
	    \EndFor
	    \State Return $Y$
	\end{algorithmic}	
\end{algorithm}

\begin{observation}\label{complete-aloc}
    All the chores in $M$ are allocated in $Y$.
\end{observation}
\begin{proof}
    All the chores that are the parent of some agent in $T$ are allocated in $Y$. Note that the leaf chores in $T$ are fully allocated to their parent in $x$ and all the fully allocated chores are also allocated in $Y$. Hence, all the chores are allocated in $Y$.
\end{proof}

\begin{observation} \label{charity}
    The number of copied chores in $Y$ is at most $n-1$.
\end{observation}
\begin{proof}
    All the chores that are integrally allocated to some agent in $x$ are allocated to one agent in $Y$ as well. Consider the step that we allocate chores to agent $i$ when iterating on $T$ in breadth-first order. Note that except $c_i$, all the chores that we allocate to $i$ are her children nodes. Since we run BFS on $T$, these children chores had not been assigned to any other agent before. Therefore, for each non-root agent, we might need to copy one chore and namely her parent node. Thus, the number of copied chores is at most $n-1$.
\end{proof}

\begin{observation}\label{lower-1}
    For all agents $i$, $p(Y_i) \geq 1$.
\end{observation}
\begin{proof}
    Since $\langle x, p \rangle$ is a CEEI, $p(x_i) = 1$ for all $i \in [n]$. Therefore, for all $i \in [n]$, $p(X_i) \geq 1$. For each agent $i$, we have $X_i = \{c \in M | 0 < x_{i,c} < 1\} \cup \{c \in M | x_{i,c} = 1\}$. Note that in $Y$ all the chores in $\{c \in M | x_{i,c} = 1\}$ are allocated to $i$. Moreover, all the chores in $\{c \in M | 0 < x_{i,c} < 1\}$ are either children of $i$ in $T$ or her parent node. In either of the cases, as long as $p(Y_i) < 1$, we add these chores to $Y_i$. If we stop before adding the whole chores in $X_i$ to $Y_i$, it means that the condition $p(Y_i) \geq 1$ is satisfied. Otherwise we have $Y_i = X_i$ and thus, $p(Y_i) \geq 1$.
\end{proof}

\begin{observation}\label{upper-1}
    For all agents $i$, there exists a chore $c$ such that $p(Y_i \setminus c) < 1$.
\end{observation}
\begin{proof}
    For all $i \in [n]$, let $X'_i$ be the set of chores integrally allocated to agent $i$ in $x$. Note that $p(X'_i) \leq p(x_i) = 1$. Hence $p((X'_i \cup c_i) \setminus c_i) \leq 1$. In other words, after the step of possibly adding $c_i$ to $Y_i$, the condition of the observation holds. Let $c$ be the last chore added to $Y_i$. Since we stop adding chores to $Y_i$ the moment $p(Y_i) > 1$, $p(Y_i \setminus c) < 1$.
\end{proof}

\begin{corollary}[of Observations \ref{lower-1} and \ref{upper-1}]\label{pef1}
    Allocation $Y$ is pEF1.
\end{corollary}

Now we are ready to prove Theorem \ref{existence}.
\existence*
\begin{proof}
    Let $Y$ be the output of Algorithm \ref{existence-alg}. Let $M'$ be the set of copied chores that are allocated in $Y$ in addition to the chores in $M$. First we prove that $\langle Y, p \rangle$ is a Fisher equilibrium for the market given by $\langle [n], M \cup M', \mathcal{D}, (p(Y_1), \ldots, p(Y_n)) \rangle$. By Observation \ref{complete-aloc}, the market clears. Since $\langle x, p \rangle$ is a CEEI for $\langle [n], M, \mathcal{D} \rangle$, for each agent $i$, all the chores in $X_i = \{ c \in M | x_{i,c} > 0 \}$ are MPB chores. Since $Y_i \subseteq X_i$, all the chores in $Y_i$ are also MPB chores. In the end, it is clear that each agent $i$ earns $p(Y_i)$. So all the conditions of a Fisher equilibrium hold for $\langle Y, p \rangle$.  Now we prove each of the properties for $Y$ separately.
    \paragraph{EF1} By Corollary \ref{pef1}, $Y$ is pEF1. Since $\langle Y, p \rangle$ is a Fisher equilibrium, Proposition \ref{pef1-prop} implies that $Y$ is EF1 too. 
    \paragraph{fPO} By Proposition \ref{PO-prop}, every Fisher equilibrium is fPO. 
    \paragraph{$(n-1)$ charity} By Observation \ref{complete-aloc}, all the chores in $M$ are allocated and by Observation \ref{charity}, the size of the charity is at most $n-1$. 
\end{proof}

\subsection{Polynomial Time Algorithm}
In this section, we prove Theorem \ref{polytime-thm}.
\polythm*
Note that the only step in Algorithm \ref{existence-alg} that is not polynomial is computing the exact CEEI. However, we can start with an approximate CEEI which is computable in polynomial time \cite{BoodaghiansCM22, combinatorial}. If we run the Algorithm \ref{existence-alg}, starting from a $(1 - \frac{1}{\den})$-CEEI, the guarantees we get in the end is that for each agent $i$, $p(Y_i) \geq (1 - \frac{1}{\den})$ and $p(Y_i \setminus c) \leq 1 + \frac{1}{\den}$ for some $c \in Y_i$.  For all agents $i$, let $h_i$ be the most expensive chore in $Y_i$. For all agents $i$ except the one with maximum income, if $p(Y_i) < 1 + \frac{1}{\den}$, add a copy of $h_i$ to $Y_i$. The pseudocode of our algorithm is shown in Algorithm \ref{poly-alg}.  

\begin{algorithm} 
	\caption{EF1 + fPO + $2(n-1)$ charity} \label{poly-alg}
	\begin{algorithmic}
	    \State Input : Instance $\mathcal{I} = ([n], M, \mathcal{D})$
	    \State Output: Allocation $Y$ 
	
	    \State $\langle x, p \rangle \leftarrow (1 - \frac{1}{\den})$-CEEI($\mathcal{I}$)
	    \State $X \leftarrow $ Output of Algorithm \ref{existence-alg} starting from $\langle x, p \rangle$
	    \State Let $p(X_1) \leq p(X_2) \leq \ldots \leq p(X_n)$
	    \For{$i \in [n-1]$}
	        \State $h_i \leftarrow$ a new copy of $\mathit{argmax}_{c \in X_i} p(c)$
	        \If{$p(X_i) < 1 + \frac{1}{\den}$}
	            \State $X_i \leftarrow X_i \cup h_i$
	        \EndIf
	    \EndFor
	    \State Return $X$
	\end{algorithmic}	
\end{algorithm}

By the exact same argument as before the final allocation is fractionally Pareto optimal and admits a Fisher equilibrium. Also the number of copied chores increases by $n-1$. Thus the total charity is at most $2(n-1)$. It only remains to prove that the final allocation is pEF1. In the rest of this section, we assume $X$ is the output of Algorithm \ref{poly-alg} and $p$ is the payment vector in Algorithm \ref{poly-alg} such that $p(X_1) \le \dots \le p(X_n)$. Next, we show that $X$ is pEF1.

\begin{observation}\label{lower-2}
    For all agents $i \in [n-1]$, $p(X_i) \geq 1+\frac{1}{\den}$.
\end{observation}
\begin{proof}
    Let $Y$ be the output of Algorithm \ref{existence-alg} starting from a $(1 - \frac{1}{\den})$-CEEI $\langle x, p \rangle$. If $p(Y_i) < 1 + \frac{1}{\den}$, we have $X_i = Y_i \cup h_i$. Note that $h_i = \mathit{argmax}_{c \in X_i} p(c)$. Therefore, $p(h_i)$ is at least the average price of the chores in $Y_i$. Hence $p(h_i) \geq (1 - \frac{1}{\den})/m$. Thus, 
    \begin{align*}
        p(X_i) &= P(Y_i \cup h_i) \\
        &\geq (1 - \frac{1}{\den}) (1+\frac{1}{m}) \\
        &\geq (1 + \frac{1}{\den})
    \end{align*}
\end{proof}

\begin{observation}\label{upper-2}
    For all agents $i$, there exists a chore $c$ such that $p(X_i \setminus c) < 1 + \frac{1}{\den}$.
\end{observation}

Now Observation \ref{lower-2} and \ref{upper-2} prove that for all $i \in [n-1]$ no agent envies the payment of agent $i$ after the removal of one chore. Also note that $p(Y_n) \geq p(X_i \setminus h_i)$ for all $i \in [n-1]$. Thus, no agent envies the payment of agent $n$ after the removal of one chore either. Therefore, $X$ is pEF1.




